An Algorithmic Pipeline for Solving Equations over Discrete Dynamical Systems Modelling Hypothesis on Real Phenomena

This paper provides an algorithmic pipeline for studying the intrinsic structure of a finite discrete dynamical system (DDS) modelling an evolving phenomenon. Here, by intrinsic structure we mean, regarding the dynamics of the DDS under observation, the feature of resulting from the "cooperation" of the dynamics of two or more smaller DDS. The intrinsic structure is described by an equation over DDS which represents a hypothesis over the phenomenon under observation. The pipeline allows solving such an equation, i.e., validating the hypothesis over the phenomenon, as far the asymptotic behavior and the number of states of the DDS under observation are concerned. The results are about the soundness and completeness of the pipeline and they are obtained by exploiting the algebraic setting for DDS introduced in [10].

==> tikzlibraryoodgraph.code.tex <==
%
% OODGraph: One Out-Degree Graphs library
%
% This library draws connected graphs with out-degree one. To draw unconnected OOD graphs, just draw separatedly their connected components
%
%\RequirePackage{etoolbox}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% This code below have been borrowed from etoolbox package  ----|          %
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%V% % % %
\newcommand*{\oodgraph@csxdef}[2]{\expandafter\xdef\csname#1\endcsname{#2}}
\newcommand*{\oodgraph@ifcsdef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}
\newcommand*{\oodgraph@ifcsundef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\expandafter
      \expandafter\@firstoftwo
    \else
      \expandafter\expandafter
      \expandafter\@secondoftwo
    \fi
  \else
    \expandafter\@firstoftwo
  \fi}
\newcommand*{\oodgraph@csuse}[1]{%
  \ifcsname#1\endcsname
    \csname#1\expandafter\endcsname
  \fi}
\newcommand{\oodgraph@cslet}[2]{%
    \expandafter\let\csname#1\endcsname#2}
\newcommand*{\oodgraph@csgundef}[1]{\global\oodgraph@cslet{#1}\relax}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % A %
% The above code have been borrowed from etoolbox package  ----| %
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%
% Version 0.1 (2019/05/25):
% - first public release
% Version 0.2 (2019/06/01):
% - added /.store in key
% - added /.default key
% - cleaned up code
% Version 0.3 (2019/06/14)
% - fixed drawing algorithm
% - points definitions are now saved in a list
% - the points list is emptied at the closing of the environment oodgraph
% Version 0.4 (2019/06/18)
% - now commands are completely scoped
% - redisigned the graph printing algorithm to take into account that now
%    everything is scoped
% Version 0.45 (2019/06/19)
% - added the option 'rotation angle'
% Version 0.46 (2019/06/20)
% - added the option 'node content'
% - added bridge to tikz and pgf when a key is not known
% - made the library independent of 'etoolbox' package (borrow
%    some code from the package)
% - added oodgraph@ prefix to all commands so to avoid conflicts with other
%    packages/libraries
% Version 0.47 (2019/06/28)
% - options 'oodgraph arrow' and 'oodgraph node' renamed into 'oodgraph edges' and 'oodgraph nodes' for more consistancy
% - fixed a bug with edges style
% - now '->' is the default edge style
% Version 0.48 (2019/07/14)
% - added a check in \addorigin to verifiy if the point has been defined before
% - some code polishing (eliminated the list oodgraph@more@options which is no
%    more used, deleted \oodgraph@resetkeys function and integrated its code
%    directly into the calling functions since its body contained only an \end{scope}
%    command, deleted several unuseful \expandafter commands)
% - explicited the definition of oodgraph@csxdef
% - partially rewritten the drawing routine for beards. Now it is much faster
% Version 0.50 (2019/07/15)
% - renamed style options 'oodgraph nodes' into 'nodes style' which is shorter and nicer
% - renamed style options 'oodgraph nodes' into 'nodes style' which is shorter and nicer
% - introduced the option 'loop style' which allows to style the loops
% - fixed a bug for the special case of cycles of order 2 which drawn the two edges
%   one over the other (obtening a double arrow). Thanks to François Doré for signalling
%   this.
% - bug fix: the beards to be wrongly oriented when the xshift key
%   was used in the addcycle command. Bug discovery and fix by François Doré
% - bug fix: when a cycle had only 2 nodes, they addresses where exchanged. Thanks
%   to François Doré for signalling this

\def\fileversion{0.50}
\def\filedate{2019/08/21}
\message{Library OODGraph}
\message{ v.\ \fileversion, \filedate}
% load tikz dependencies
\usetikzlibrary{calc}
\makeatletter
\gdef\oodgraph@tmp{}
\gdef\oodgraph@points@list{}
%
% convenience routines to extract the prefix from a node path
%
\def\oodgraph@get@prefix@from@path@@#1-#2\pgf@eov{\xdef\oodgraph@tmp{\oodgraph@csuse{#1.origin}}}
\def\oodgraph@get@prefix@from@path#1{
\pgfutil@in@{-}{#1}
\ifpgfutil@in@% if there is a minus sign then it is a package defined point
\oodgraph@get@prefix@from@path@@#1\pgf@eov
\else% regular pgf/tikz point
\path(#1);\pgfgetlastxy{\XCoord}{\YCoord};
\xdef\oodgraph@tmp{(\XCoord,\YCoord)}
\fi
}
%
%  oodgraph@addtolist
%  #1 = name of the list to add to
%  #2 = object to be added
% Service function to append objects to lists
%
\newcommand*{\oodgraph@addtolist}[2]{%
   \expandafter\if\expandafter\relax\csname #1\endcsname\relax%
      \expandafter\expandafter\xdef\csname #1\endcsname{#2}%
   \else%
    \expandafter\xdef\csname #1\endcsname{\csname #1\endcsname,#2}%
\fi%
}
%
%  oodgraph@docslist@undeft
%  #1 = separator char
%  #2 = name of the list
% Service routine to \csundef all elements of the list
% 
\newcommand{\oodgraph@docslist@undef}[2][,]{%
%   #1 = separation char
%   #2 = list
   \def\dolist##1{\expandafter\@dolist##1#1\@eol}%
   \def\@dolist##1#1##2\@eol{%
   % process stuff here with ##1
   \oodgraph@csgundef{##1}
   \ifx\@eol##2\@eol\else\@dolist##2\@eol\fi}%
   \dolist{#2}%
}
%
\pgfkeys{/oodgraph/.search also={/tikz, /pgf}} %,/oodgraph/catch unknown}}%
%\pgfkeys{/oodgraph/.search also={/tikz,/pgf,/oodgraph/catch unknown}}%
\pgfkeys{%
/oodgraph/.cd,
%radius/.initial={1},
radius/.value required,
radius/.default={1},
radius/.store in=\oodgraph@radius,
radius,
%attach node/.initial={a->1},
attach node/.value required,
attach node/.default={a->1},
attach node/.store in=\oodgraph@attach@node,
attach node,
%nodes prefix/.initial={a},
nodes prefix/.value required,
nodes prefix/.default={a},
nodes prefix/.store in=\oodgraph@nodes@prefix,
nodes prefix,
%opening angle/.initial={120},
opening angle/.value required,
opening angle/.default={120},
opening angle/.store in=\oodgraph@opa,
opening angle,
rotation angle/.value required,
rotation angle/.default={0},
rotation angle/.store in=\oodgraph@rota,
rotation angle,
nodes content/.value required,
nodes content/.default={$\bullet$},
nodes content/.store in=\oodgraph@node@content,
nodes content,
nodes@style/.style={},
edges@style/.style={->},
loop@style/.style={out=-30, in=-150,looseness=6},
nodes style/.code=\pgfkeys{/oodgraph/nodes@style/.style={#1}},
edges style/.code=\pgfkeys{/oodgraph/edges@style/.style={#1}},
loop style/.code=\pgfkeys{/oodgraph/loop@style/.style={#1}},
semi thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={semi thick}},
thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={thick}},
ultra thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={ultra thick}},
edges color/.code=\pgfkeys{/oodgraph/edges@style/.append style={#1}},
nodes color/.code=\pgfkeys{/oodgraph/nodes@style/.append style={#1}},
}
%\pgfkeys{/oodgraph/.unknown/.code={%
%\ifx#1\pgfutil@empty\oodgraph@addtolist{oodgraph@more@options}{\pgfkeyscurrentname}\else\oodgraph@addtolist{oodgraph@more@options}{\pgfkeyscurrentname=#1}
%\fi}}
%
\newenvironment{oodgraph}[1][]{\begin{scope}[#1]}
{% closing the environment
% free all points definition in the current list
%\forcsvlist{\csgundef}{\oodgraph@points@list}
\expandafter\oodgraph@docslist@undef\expandafter{\oodgraph@points@list}
% free the points list
\gdef\oodgraph@points@list{}
% free temporary definitions
\gdef\oodgraph@tmp{}
\end{scope}}
%
\newcommand{\oodgraph@processkeys}[1][]{
\begin{scope}
\pgfkeys{/oodgraph/.cd,#1}
}
\long\def\oodgraph@drawcycle#1;{
\ifnum#1=1\oodgraph@drawcycle@\else%
{\ifnum#1=2\oodgraph@drawcycle@@{#1}\else%
\oodgraph@drawcycle@@@{#1}\fi}\fi
% record circle center on points list and define it
\path(0,0);\pgfgetlastxy{\XCoord}{\YCoord};
\oodgraph@ifcsundef{\oodgraph@nodes@prefix.origin}{%
% if undefined then add to the point list
\oodgraph@csxdef{\oodgraph@nodes@prefix.origin}{(\XCoord,\YCoord)}
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix.origin}
}%
{% if already defined then simply replace the old definition
\oodgraph@csxdef{\oodgraph@nodes@prefix.origin}{(\XCoord,\YCoord)}
}%
\end{scope}
}
%
\newcommand{\oodgraph@drawcycle@}{
%\pgfcoordinate{myorigin}{\pgfpointorigin}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->1) at(0,0){\oodgraph@node@content};
% save points on the list
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->1}
%\expandafter\oodgraph@csxdef\expandafter{\oodgraph@nodes@prefix->1}{(0pt,0pt)}
\oodgraph@csxdef{\oodgraph@nodes@prefix->1}{(0pt,0pt)}
% draw edges
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->1) edge[/oodgraph/loop@style] (\oodgraph@nodes@prefix->1);
}
\newcommand{\oodgraph@drawcycle@@}{
% second node
\pgfmathsetmacro{\oodgraph@half@radius}{.5*\oodgraph@radius}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->2) at(-\oodgraph@half@radius,0){\oodgraph@node@content};
% first node
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->1) at(\oodgraph@half@radius,0){\oodgraph@node@content};
% register nodes
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->1}
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->2}
\oodgraph@csxdef{\oodgraph@nodes@prefix->1}{(-\oodgraph@half@radius,0pt)}
\oodgraph@csxdef{\oodgraph@nodes@prefix->2}{(\oodgraph@half@radius,0pt)}
% draw edges
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->1) edge[/oodgraph/edges@style, bend left] (\oodgraph@nodes@prefix->2);
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->2) edge[/oodgraph/edges@style, bend left] (\oodgraph@nodes@prefix->1);
}
\newcommand{\oodgraph@drawcycle@@@}[1]{
\pgfmathsetmacro\myangle{360.0/#1}
\foreach \i in {1,...,#1}{
  \pgfmathsetmacro\curangle{(\i-1)*\myangle}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->\i) at ({\oodgraph@radius*cos(\curangle)},{\oodgraph@radius*sin(\curangle)}){\oodgraph@node@content};
  \path(\oodgraph@nodes@prefix->\i); \pgfgetlastxy{\XCoord}{\YCoord};
  \oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->\i}
  \oodgraph@csxdef{\oodgraph@nodes@prefix->\i}{(\XCoord,\YCoord)}
}
%\wlog{list=\oodgraph@points@list}
\foreach \i in {1,...,#1}{
  \pgfmathsetmacro\mynext{ifthenelse(\i==#1,int(1),int(\i+1))}
  \draw[/oodgraph/edges@style] (\oodgraph@nodes@prefix->\i) -- (\oodgraph@nodes@prefix->\mynext);
}
}
\newcommand*{\addcycle}[1][]{%
\oodgraph@processkeys[#1]
\oodgraph@drawcycle
}
%
\def\addorigin#1;{%
\pgfutil@ifundefined{pgf@sh@ns@#1}{
\edef\mymsgtmp{No point named #1\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the point has been correctly defined via the standard TikZ interface.}
}{%
\path(#1);\pgfgetlastxy{\XCoord}{\YCoord};
\oodgraph@csxdef{#1}{(\XCoord,\YCoord)}%
\oodgraph@csxdef{#1.origin}{(\XCoord,\YCoord)}%
%\oodgraph@addtolist{oodgraph@points@list}{#1} % added v. 0.48
%\oodgraph@addtolist{oodgraph@points@list}{#1.origin} % added v. 0.48
}}
%
\newcommand{\addbeard}[1][]{%
\oodgraph@processkeys[#1]
\oodgraph@drawbeardlev
}
\def\oodgraph@drawbeardlev#1;{%
%\wlog{list=\oodgraph@points@list}
\ifnum#1=1\oodgraph@drawbeardlev@\else\oodgraph@drawbeardlev@@{#1}\fi
\end{scope}}
\newcommand{\oodgraph@drawbeardlev@}{
\oodgraph@ifcsdef{\oodgraph@attach@node}{%
\expandafter\oodgraph@get@prefix@from@path\expandafter{\oodgraph@attach@node}
\path[reset cm]\oodgraph@tmp;\pgfgetlastxy{\XOCoord}{\YOCoord};
%\path[reset cm]\oodgraph@csuse{\oodgraph@attach@node};\pgfgetlastxy{\XCoord}{\YCoord};
\path[reset cm](\oodgraph@attach@node);\pgfgetlastxy{\XCoord}{\YCoord};
}{% else signal errors
\edef\mymsgtmp{No point named \oodgrap@attach@node\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the attachment node has been correctly defined or that there exists
a addorigin command.}
}%
\begin{scope}[shift={(\XOCoord, \YOCoord)}]
% recompute the coordinates of attach point in the new coordinate system
\pgfmathsetmacro\XCoord{\XCoord-\XOCoord}
\pgfmathsetmacro\YCoord{\YCoord-\YOCoord}
% compute angle wrt attachment point
\pgfmathsetmacro\myalphatmp{atan(\YCoord/(\XCoord+.01))}
\pgfmathsetmacro\myalpha{ifthenelse(\XCoord>=0,\myalphatmp,180+\myalphatmp)}
\pgfmathsetmacro\myalpha{\myalpha+\oodgraph@rota}
%
% draw the new node
\node[/oodgraph/nodes@style](\oodgraph@attach@node->1) at ($(\oodgraph@attach@node)+({\oodgraph@radius*cos(\myalpha)},{\oodgraph@radius*sin(\myalpha)})$){\oodgraph@node@content};
\draw[/oodgraph/edges@style] (\oodgraph@attach@node->1) -- (\oodgraph@attach@node);
% store infos about node
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@attach@node->1}
\path(\oodgraph@attach@node->1); \pgfgetlastxy{\XCoord}{\YCoord};
\oodgraph@csxdef{\oodgraph@attach@node->1}{(\XCoord,\YCoord)}
\end{scope}
}
\newcommand{\oodgraph@drawbeardlev@@}[1]{
% #1= number of nodes in the level
% check if the attachment node has been previously defined
\oodgraph@ifcsdef{\oodgraph@attach@node}{% then part
% if the attach node has been defined then
% find the root prefix and retrive the origin
\expandafter\oodgraph@get@prefix@from@path\expandafter{\oodgraph@attach@node}
\path[reset cm]\oodgraph@tmp;\pgfgetlastxy{\XOCoord}{\YOCoord};
\path[reset cm](\oodgraph@attach@node);\pgfgetlastxy{\XCoord}{\YCoord};
}% end of then part
{% if it is not defined, print an error message
\edef\mymsgtmp{No point named \oodgrap@attach@node\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the attachment node has been correctly defined or that there exists a addorigin command.}
}%
\begin{scope}[shift={(\XOCoord, \YOCoord)}]
% myangle = angle between two successive points of the beard level
\pgfmathsetmacro\myangle{\oodgraph@opa/#1}
% recompute coordinates of attach point in the new coordinate system
\pgfmathsetmacro\XCoord{\XCoord-\XOCoord}
\pgfmathsetmacro\YCoord{\YCoord-\YOCoord}
% compute angle wrt attachment point
\pgfmathsetmacro\myalphatmp{atan(\YCoord/(\XCoord+.01))}
\pgfmathsetmacro\myalpha{ifthenelse(\XCoord>=0,\myalphatmp,180+\myalphatmp)}
\pgfmathsetmacro\myalpha{\myalpha+\oodgraph@rota}
% compute the offset angle
\pgfmathsetmacro\myofsangle{ifthenelse(mod(#1,2)==1,0.0,\myangle/2.0}
% draw nodes and edges
%\node at (6,6.5){alpha corr=\myalphacorr};
%\node at (6,6){\oodgraph@attach@node=\csuse{\oodgraph@attach@node}};
%\node at (6,5){point=(\XCoord,\YCoord)};
%\node at (6,4.5){myalpha=\myalpha};
%\node at (6,4.5){myangle=\myangle};
%\node at (6,4){myofsangle=\myofsangle};
%\node at (6,3.5){myend=\myend};
\pgfmathsetmacro\myend{int(ceil(#1/2.0))}
\pgfmathsetmacro\myalpha{\myalpha+\myend*\myangle+2*\myofsangle}
\foreach \i in {#1,...,1}{
\pgfmathsetmacro\mycurangle{\myalpha-(#1-\i+1)*\myangle-\myofsangle}
%\node at (6,3.5-\i){mycurangle=\mycurangle};
\node[/oodgraph/nodes@style](\oodgraph@attach@node->\i) at ($(\oodgraph@attach@node)+({\oodgraph@radius*cos(\mycurangle)},{\oodgraph@radius*sin(\mycurangle)})$){\oodgraph@node@content};
  \draw[/oodgraph/edges@style] (\oodgraph@attach@node->\i) -- (\oodgraph@attach@node);
  % save points to points@list
  \path(\oodgraph@attach@node->\i); \pgfgetlastxy{\XCoord}{\YCoord};
 \oodgraph@addtolist{oodgraph@points@list}{\oodgraph@attach@node->\i}
 \oodgraph@csxdef{\oodgraph@attach@node->\i}{(\XCoord,\YCoord)}
}
\end{scope}}
%
\makeatother
%
\endinput
